Towards Deterministic Algorithms for Constant-Depth Factors of Constant-Depth Circuits

We design a deterministic subexponential time algorithm that takes as input a multivariate polynomial $f$ computed by a constant-depth circuit over rational numbers, and outputs a list $L$ of circuits (of unbounded depth and possibly with division gates) that contains all irreducible factors of $f$ computable by constant-depth circuits. This list $L$ might also include circuits that are spurious: they either do not correspond to factors of $f$ or are not even well-defined, e.g. the input to a division gate is a sub-circuit that computes the identically zero polynomial. The key technical ingredient of our algorithm is a notion of the pseudo-resultant of $f$ and a factor $g$, which serves as a proxy for the resultant of $g$ and $f/g$, with the advantage that the circuit complexity of the pseudo-resultant is comparable to that of the circuit complexity of $f$ and $g$. This notion, which might be of independent interest, together with the recent results of Limaye, Srinivasan and Tavenas, helps us derandomize one key step of multivariate polynomial factorization algorithms - that of deterministically finding a good starting point for Newton Iteration for the case when the input polynomial as well as the irreducible factor of interest have small constant-depth circuits.

==> hooks/post-checkout <==
#!/bin/sh
# Copyright 2011 Brent Longborough
# Please read gitinfo.pdf for licencing and other details
# -----------------------------------------------------
# Post-{commit,checkout,merge} hook for the gitinfo package
#
prefixes=". test docs"    # Example for multiple gitHeadInfo.tex files
prefixes="."              # Default --- in the working copy root
for pref in $prefixes
	do
	git log -1 --date=short \
	--pretty=format:"\usepackage[%
		shash={%h},
		lhash={%H},
		authname={%an},
		authemail={%ae},
		authsdate={%ad},
		authidate={%ai},
		authudate={%at},
		commname={%an},
		commemail={%ae},
		commsdate={%ad},
		commidate={%ai},
		commudate={%at},
		refnames={%d}
	]{gitsetinfo}" HEAD > $pref/gitHeadInfo.gin
	done


==> hooks/post-commit <==
#!/bin/sh
# Copyright 2011 Brent Longborough
# Please read gitinfo.pdf for licencing and other details
# -----------------------------------------------------
# Post-{commit,checkout,merge} hook for the gitinfo package
#
# prefixes=". test docs"    # Example for multiple gitHeadInfo.tex files
prefixes="."              # Default --- in the working copy root
for pref in $prefixes
	do
	git log -1 --date=short \
	--pretty=format:"\usepackage[%
		shash={%h},
		lhash={%H},
		authname={%an},
		authemail={%ae},
		authsdate={%ad},
		authidate={%ai},
		authudate={%at},
		commname={%an},
		commemail={%ae},
		commsdate={%ad},
		commidate={%ai},
		commudate={%at},
		refnames={%d}
	]{gitsetinfo}" HEAD > $pref/gitHeadInfo.gin
	done


==> hooks/post-merge <==
#!/bin/sh
# Copyright 2011 Brent Longborough
# Please read gitinfo.pdf for licencing and other details
# -----------------------------------------------------
# Post-{commit,checkout,merge} hook for the gitinfo package
#
# prefixes=". test docs"    # Example for multiple gitHeadInfo.tex files
prefixes="."              # Default --- in the working copy root
for pref in $prefixes
	do
	git log -1 --date=short \
	--pretty=format:"\usepackage[%
		shash={%h},
		lhash={%H},
		authname={%an},
		authemail={%ae},
		authsdate={%ad},
		authidate={%ai},
		authudate={%at},
		commname={%an},
		commemail={%ae},
		commsdate={%ad},
		commidate={%ai},
		commudate={%at},
		refnames={%d}
	]{gitsetinfo}" HEAD > $pref/gitHeadInfo.gin
	done

